Adversarial Examples and Metrics

Adversarial examples are a type of attack on machine learning (ML) systems which cause misclassification of inputs. Achieving robustness against adversarial examples is crucial to apply ML in the real world. While most prior work on adversarial examples is empirical, a recent line of work establishes fundamental limitations of robust classification based on cryptographic hardness. Most positive and negative results in this field however assume that there is a fixed target metric which constrains the adversary, and we argue that this is often an unrealistic assumption. In this work we study the limitations of robust classification if the target metric is uncertain. Concretely, we construct a classification problem, which admits robust classification by a small classifier if the target metric is known at the time the model is trained, but for which robust classification is impossible for small classifiers if the target metric is chosen after the fact. In the process, we explore a novel connection between hardness of robust classification and bounded storage model cryptography.

==> gnuplot-lua-tikz-common.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%     Common style file for TeX, LaTeX and ConTeXt
%%  
%%  It is associated with the 'gnuplot.lua' script, and usually generated
%%  automatically. So take care whenever you make any changes!
%%

% check for the correct TikZ version
\def\gpchecktikzversion#1.#2\relax{%
\ifnum#1<2%
  \errmessage{PGF/TikZ version >= 2.0 is required!}%
\fi}
\expandafter\gpchecktikzversion\pgfversion\relax

% FIXME: is there a more elegant way to determine the output format?

\def\pgfsysdriver@a{pgfsys-dvi.def}       % ps
\def\pgfsysdriver@b{pgfsys-dvipdfm.def}   % pdf
\def\pgfsysdriver@c{pgfsys-dvipdfmx.def}  % pdf
\def\pgfsysdriver@d{pgfsys-dvips.def}     % ps
\def\pgfsysdriver@e{pgfsys-pdftex.def}    % pdf
\def\pgfsysdriver@f{pgfsys-tex4ht.def}    % html
\def\pgfsysdriver@g{pgfsys-textures.def}  % ps
\def\pgfsysdriver@h{pgfsys-vtex.def}      % ps
\def\pgfsysdriver@i{pgfsys-xetex.def}     % pdf

\newif\ifgppdfout\gppdfoutfalse
\newif\ifgppsout\gppsoutfalse

\ifx\pgfsysdriver\pgfsysdriver@a
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@b
  \gppdfouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@c
  \gppdfouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@d
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@e
  \gppdfouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@f
  % tex4ht
\else\ifx\pgfsysdriver\pgfsysdriver@g
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@h
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@i
  \gppdfouttrue
\fi\fi\fi\fi\fi\fi\fi\fi\fi

% uncomment the following lines to make font values "appendable"
% and if you are really sure about that ;-)
% \pgfkeyslet{/tikz/font/.@cmd}{\undefined}
% \tikzset{font/.initial={}}
% \def\tikz@textfont{\pgfkeysvalueof{/tikz/font}}

%
% image related stuff
%
\def\gp@rawimage@pdf#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{/CMYK}%
  \else%
    \def\gp@temp{/RGB}%
  \fi%
  \pgf@sys@bp{#4}\pgfsysprotocol@literalbuffered{0 0}\pgf@sys@bp{#5}%
  \pgfsysprotocol@literalbuffered{0 0 cm}%
  \pgfsysprotocol@literalbuffered{BI /W #2 /H #3 /CS \gp@temp}%
  \pgfsysprotocol@literalbuffered{/BPC 8 /F /AHx ID}%
  \pgfsysprotocol@literal{#6 > EI}%
}
\def\gp@rawimage@ps#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{4}%
  \else%
    \def\gp@temp{3}%
  \fi%
  \pgfsysprotocol@literalbuffered{0 0 translate}%
  \pgf@sys@bp{#4}\pgf@sys@bp{#5}\pgfsysprotocol@literalbuffered{scale}%
  \pgfsysprotocol@literalbuffered{#2 #3 8 [#2 0 0 -#3 0 #3]}%
  \pgfsysprotocol@literalbuffered{currentfile /ASCIIHexDecode filter}%
  \pgfsysprotocol@literalbuffered{false \gp@temp\space colorimage}%
  \pgfsysprotocol@literal{#6 >}%
}
\def\gp@rawimage@html#1#2#3#4#5#6{%
% FIXME: print a warning message here
}

\ifgppdfout
  \def\gp@rawimage{\gp@rawimage@pdf}
\else
  \ifgppsout
    \def\gp@rawimage{\gp@rawimage@ps}
  \else
    \def\gp@rawimage{\gp@rawimage@html}
  \fi
\fi


\def\gploadimage#1#2#3#4#5{%
  \pgftext[left,bottom,x=#1cm,y=#2cm] {\pgfimage[interpolate=false,width=#3cm,height=#4cm]{#5}};%
}

\def\gp@set@size#1{%
  \def\gp@image@size{#1}%
}

\def\gp@rawimage@#1#2#3#4#5#6#7#8{
  \tikz@scan@one@point\gp@set@size(#6,#7)\relax%
  \tikz@scan@one@point\pgftransformshift(#2,#3)\relax%
  \pgftext {%
    \pgfsys@beginpurepicture%
    \gp@image@size% fill \pgf@x and \pgf@y
    \gp@rawimage{#1}{#4}{#5}{\pgf@x}{\pgf@y}{#8}%
    \pgfsys@endpurepicture%
  }%
}

%% \gprawimage{color model}{xcoord}{ycoord}{# of xpixel}{# of ypixel}{xsize}{ysize}{rgb/cmyk hex data RRGGBB/CCMMYYKK ...}{file name}
%% color model is 'cmyk' or 'rgb' (default)
\def\gprawimage#1#2#3#4#5#6#7#8#9{%
  \ifx&#9&%
    \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}
  \else
    \ifgppsout
      \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}
    \else
      \gploadimage{#2}{#3}{#6}{#7}{#9}
    \fi
  \fi
}

%
% gnuplottex comapatibility
% (see http://www.ctan.org/tex-archive/help/Catalogue/entries/gnuplottex.html)
%

\def\gnuplottexextension@lua{\string tex}
\def\gnuplottexextension@tikz{\string tex}

%
% gnuplot variables getter and setter
%

\def\gpsetvar#1#2{%
  \expandafter\xdef\csname gp@var@#1\endcsname{#2}
}

\def\gpgetvar#1{%
  \csname gp@var@#1\endcsname %
}

%
% some wrapper code
%

% short for a filled path
\def\gpfill#1{\path[line width=0.1\gpbaselw,draw,fill,#1]}

% short for changing the line width
\def\gpsetlinewidth#1{\pgfsetlinewidth{#1\gpbaselw}}

% short for changing the line type
\def\gpsetlinetype#1{\tikzset{gp path/.style={#1,#1 add}}}

% short for changing the dash pattern
\def\gpsetdashtype#1{\tikzset{gp path/.append style={#1}}}

% short for changing the point size
\def\gpsetpointsize#1{\tikzset{gp point/.style={mark size=#1\gpbasems}}}

% wrapper for color settings
\def\gpcolor#1{\tikzset{global #1}}
\tikzset{rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\tikzset{color=.}}}
\tikzset{global rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\pgfutil@color{.}}}
\tikzset{global color/.code={\pgfutil@color{#1}}}

% prevent plot mark distortions due to changes in the PGF transformation matrix
% use `\gpscalepointstrue' and `\gpscalepointsfalse' for enabling and disabling
% point scaling
%
\newif\ifgpscalepoints
\tikzset{gp shift only/.style={%
  \ifgpscalepoints\else shift only\fi%
}}
\def\gppoint#1#2{%
  \path[solid] plot[only marks,gp point,mark options={gp shift only},#1] coordinates {#2};%
}


%
% char size calculation, that might be used with gnuplottex
%
% Example code (needs gnuplottex.sty):
%
%    % calculate the char size when the "gnuplot" style is used
%    \tikzset{gnuplot/.append style={execute at begin picture=\gpcalccharsize}}
%
%    \tikzset{gnuplot/.append style={font=\ttfamily\footnotesize}}
%
%    \begin{tikzpicture}[gnuplot]
%      \begin{gnuplot}[terminal=lua,%
%          terminaloptions={tikz solid nopic charsize \the\gphcharsize,\the\gpvcharsize}]
%        test
%      \end{gnuplot}
%    \end{tikzpicture}
%
%%%
% The `\gpcalccharsize' command fills the lengths \gpvcharsize and \gphcharsize with
% the values of the current default font used within nodes and is meant to be called
% within a tikzpicture environment.
% 
\newdimen\gpvcharsize
\newdimen\gphcharsize
\def\gpcalccharsize{%
  \pgfinterruptboundingbox%
  \pgfsys@begininvisible%
  \node at (0,0) {%
    \global\gphcharsize=1.05\fontcharwd\font`0%
    \global\gpvcharsize=1.05\fontcharht\font`0%
    \global\advance\gpvcharsize by 1.05\fontchardp\font`g%
  };%
  \pgfsys@endinvisible%
  \endpgfinterruptboundingbox%
}

%
%  define a rectangular node in tikz e.g. for the plot area
%
%  #1 node name
%  #2 coordinate of "south west"
%  #3 coordinate of "north east"
%
\def\gpdefrectangularnode#1#2#3{%
  \expandafter\gdef\csname pgf@sh@ns@#1\endcsname{rectangle}
  \expandafter\gdef\csname pgf@sh@np@#1\endcsname{%
    \def\southwest{#2}%
    \def\northeast{#3}%
  }
  \pgfgettransform\pgf@temp%
  % once it is defined, no more transformations will be applied, I hope
  \expandafter\xdef\csname pgf@sh@nt@#1\endcsname{\pgf@temp}%
  \expandafter\xdef\csname pgf@sh@pi@#1\endcsname{\pgfpictureid}%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  You may want to adapt the following to fit your needs (in your 
%%  individual style file and/or within your document).
%%

%
% style for every plot
%
\tikzset{gnuplot/.style={%
  >=stealth',%
  line cap=round,%
  line join=round,%
}}

\tikzset{gp node left/.style={anchor=mid west,yshift=-.12ex}}
\tikzset{gp node center/.style={anchor=mid,yshift=-.12ex}}
\tikzset{gp node right/.style={anchor=mid east,yshift=-.12ex}}

% basic plot mark size (points)
\newdimen\gpbasems
\gpbasems=.4pt

% basic linewidth
\newdimen\gpbaselw
\gpbaselw=.4pt

% this is the default color for pattern backgrounds
\colorlet{gpbgfillcolor}{white}

% set background color and fill color
\def\gpsetbgcolor#1{%
  \pgfutil@definecolor{gpbgfillcolor}{rgb}{#1}%
  \tikzset{tight background,background rectangle/.style={fill=gpbgfillcolor},show background rectangle}%
}

% this should reverse the normal text node presets, for the
% later referencing as described below
\tikzset{gp refnode/.style={coordinate,yshift=.12ex}}

% to add an empty label with the referenceable name "my node"
% to the plot, just add the following line to your gnuplot
% file:
%
% set label "" at 1,1 font ",gp refnode,name=my node"
%

% enlargement of the bounding box in standalone mode (only used by LaTeX/ConTeXt)
\def\gpbboxborder{0mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  The following TikZ-styles are derived from the 'pgf.styles.*' tables
%%  in the Lua script.
%%  To change the number of used styles you should change them there and
%%  regenerate this style file.
%%

% arrow styles settings
\tikzset{gp arrow 1/.style={>=latex}}
\tikzset{gp arrow 2/.style={>=angle 90}}
\tikzset{gp arrow 3/.style={>=angle 60}}
\tikzset{gp arrow 4/.style={>=angle 45}}
\tikzset{gp arrow 5/.style={>=o}}
\tikzset{gp arrow 6/.style={>=*}}
\tikzset{gp arrow 7/.style={>=diamond}}
\tikzset{gp arrow 8/.style={>=open diamond}}
\tikzset{gp arrow 9/.style={>={]}}}
\tikzset{gp arrow 10/.style={>={[}}}
\tikzset{gp arrow 11/.style={>=)}}
\tikzset{gp arrow 12/.style={>=(}}

% plotmark settings
\tikzset{gp mark 0/.style={mark size=.5\pgflinewidth,mark=*}}
\tikzset{gp mark 1/.style={mark=+}}
\tikzset{gp mark 2/.style={mark=x}}
\tikzset{gp mark 3/.style={mark=star}}
\tikzset{gp mark 4/.style={mark=square}}
\tikzset{gp mark 5/.style={mark=square*}}
\tikzset{gp mark 6/.style={mark=o}}
\tikzset{gp mark 7/.style={mark=*}}
\tikzset{gp mark 8/.style={mark=triangle}}
\tikzset{gp mark 9/.style={mark=triangle*}}
\tikzset{gp mark 10/.style={mark=triangle,every mark/.append style={rotate=180}}}
\tikzset{gp mark 11/.style={mark=triangle*,every mark/.append style={rotate=180}}}
\tikzset{gp mark 12/.style={mark=diamond}}
\tikzset{gp mark 13/.style={mark=diamond*}}
\tikzset{gp mark 14/.style={mark=otimes}}
\tikzset{gp mark 15/.style={mark=oplus}}

% pattern settings
\tikzset{gp pattern 0/.style={white}}
\tikzset{gp pattern 1/.style={pattern=north east lines}}
\tikzset{gp pattern 2/.style={pattern=north west lines}}
\tikzset{gp pattern 3/.style={pattern=crosshatch}}
\tikzset{gp pattern 4/.style={pattern=grid}}
\tikzset{gp pattern 5/.style={pattern=vertical lines}}
\tikzset{gp pattern 6/.style={pattern=horizontal lines}}
\tikzset{gp pattern 7/.style={pattern=dots}}
\tikzset{gp pattern 8/.style={pattern=crosshatch dots}}
\tikzset{gp pattern 9/.style={pattern=fivepointed stars}}
\tikzset{gp pattern 10/.style={pattern=sixpointed stars}}
\tikzset{gp pattern 11/.style={pattern=bricks}}

% if the 'tikzplot' option is used the corresponding lines will be smoothed by default
\tikzset{gp plot axes/.style=}
\tikzset{gp plot border/.style=}
\tikzset{gp plot 0/.style=smooth}
\tikzset{gp plot 1/.style=smooth}
\tikzset{gp plot 2/.style=smooth}
\tikzset{gp plot 3/.style=smooth}
\tikzset{gp plot 4/.style=smooth}
\tikzset{gp plot 5/.style=smooth}
\tikzset{gp plot 6/.style=smooth}
\tikzset{gp plot 7/.style=smooth}

% linestyle settings
\tikzset{gp lt axes/.style=dotted}
\tikzset{gp lt border/.style=solid}

% linestyle "addon" settings for overwriting a default linestyle within the
% TeX document via eg. \tikzset{gp lt plot 1 add/.style={fill=black,draw=none}} etc.
\tikzset{gp lt axes add/.style={}}
\tikzset{gp lt border add/.style={}}
\tikzset{gp lt plot 0 add/.style={}}
\tikzset{gp lt plot 1 add/.style={}}
\tikzset{gp lt plot 2 add/.style={}}
\tikzset{gp lt plot 3 add/.style={}}
\tikzset{gp lt plot 4 add/.style={}}
\tikzset{gp lt plot 5 add/.style={}}
\tikzset{gp lt plot 6 add/.style={}}
\tikzset{gp lt plot 7 add/.style={}}
\tikzset{gp lt plot 0/.style={}}
\tikzset{gp lt plot 1/.style={}}
\tikzset{gp lt plot 2/.style={}}
\tikzset{gp lt plot 3/.style={}}
\tikzset{gp lt plot 4/.style={}}
\tikzset{gp lt plot 5/.style={}}
\tikzset{gp lt plot 6/.style={}}
\tikzset{gp lt plot 7/.style={}}

% linestyle color settings
\colorlet{gp lt color axes}{black!30}
\colorlet{gp lt color border}{black}

% dash type settings
% Define this as a macro so that the dash patterns expand later with the current \pgflinewidth.
\def\gpdashlength{\pgflinewidth}
\tikzset{gp dt 0/.style={solid}}
\tikzset{gp dt 1/.style={solid}}
\tikzset{gp dt 2/.style={dash pattern=on 7.5*\gpdashlength off 7.5*\gpdashlength}}
\tikzset{gp dt 3/.style={dash pattern=on 3.75*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 4/.style={dash pattern=on 1*\gpdashlength off 2.8125*\gpdashlength}}
\tikzset{gp dt 5/.style={dash pattern=on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt 6/.style={dash pattern=on 5.625*\gpdashlength off 5.625*\gpdashlength on 1*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 7/.style={dash pattern=on 3.75*\gpdashlength off 3.75*\gpdashlength on 3.75*\gpdashlength off 11.25*\gpdashlength}}
\tikzset{gp dt 8/.style={dash pattern=on 1*\gpdashlength off 3.75*\gpdashlength on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt solid/.style={solid}}
\tikzset{gp dt axes/.style={dotted}}

% command for switching to colored lines
\def\gpcoloredlines{%
  \colorlet{gp lt color 0}{red}%
  \colorlet{gp lt color 1}{green}%
  \colorlet{gp lt color 2}{blue}%
  \colorlet{gp lt color 3}{magenta}%
  \colorlet{gp lt color 4}{cyan}%
  \colorlet{gp lt color 5}{yellow}%
  \colorlet{gp lt color 6}{orange}%
  \colorlet{gp lt color 7}{purple}%
}

% command for switching to monochrome (black) lines
\def\gpmonochromelines{%
  \colorlet{gp lt color 0}{black}%
  \colorlet{gp lt color 1}{black}%
  \colorlet{gp lt color 2}{black}%
  \colorlet{gp lt color 3}{black}%
  \colorlet{gp lt color 4}{black}%
  \colorlet{gp lt color 5}{black}%
  \colorlet{gp lt color 6}{black}%
  \colorlet{gp lt color 7}{black}%
}

%
% some initialisations
%
% by default all lines will be colored
\gpcoloredlines
\gpsetpointsize{4}
\gpsetlinetype{gp lt solid}
\gpscalepointsfalse
\endinput


==> gnuplot-lua-tikz.tex <==
%%
%%  plain TeX wrapper for gnuplot-tikz style file
%%
\input tikz.tex
\usetikzlibrary{arrows,patterns,plotmarks,backgrounds}

\edef\tikzatcode{\the\catcode`\@}
\catcode`\@=11

\input gnuplot-lua-tikz-common.tex


\catcode`\@=\tikzatcode

\endinput


==> iccv.tex <==
Adversarial Robustness vs. Model Compression, or Both?
http://openaccess.thecvf.com/content_ICCV_2019/papers/Ye_Adversarial_Robustness_vs._Model_Compression_or_Both_ICCV_2019_paper.pdf

Human Uncertainty Makes Classification More Robust
Joshua C. Peterson, Ruairidh M. Battleday, Thomas L. Griffiths, Olga Russakovsky; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 9617-9626
http://openaccess.thecvf.com/content_ICCV_2019/html/Peterson_Human_Uncertainty_Makes_Classification_More_Robust_ICCV_2019_paper.html

A Decoupled 3D Facial Shape Model by Adversarial Training
Victoria Fernandez Abrevaya, Adnane Boukhayma, Stefanie Wuhrer, Edmond Boyer; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 9419-9428
http://openaccess.thecvf.com/content_ICCV_2019/html/Abrevaya_A_Decoupled_3D_Facial_Shape_Model_by_Adversarial_Training_ICCV_2019_paper.html

advPattern: Physical-World Attacks on Deep Person Re-Identification via Adversarially Transformable Patterns
Zhibo Wang, Siyan Zheng, Mengkai Song, Qian Wang, Alireza Rahimpour, Hairong Qi; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 8341-8350
http://openaccess.thecvf.com/content_ICCV_2019/html/Wang_advPattern_Physical-World_Attacks_on_Deep_Person_Re-Identification_via_Adversarially_Transformable_ICCV_2019_paper.html

FDA: Feature Disruptive Attack
Aditya Ganeshan, Vivek B.S., R. Venkatesh Babu; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 8069-8079
http://openaccess.thecvf.com/content_ICCV_2019/html/Ganeshan_FDA_Feature_Disruptive_Attack_ICCV_2019_paper.html

Addressing Model Vulnerability to Distributional Shifts Over Image Transformation Sets
Riccardo Volpi, Vittorio Murino; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 7980-7989
http://openaccess.thecvf.com/content_ICCV_2019/html/Volpi_Addressing_Model_Vulnerability_to_Distributional_Shifts_Over_Image_Transformation_Sets_ICCV_2019_paper.html

Attributing Fake Images to GANs: Learning and Analyzing GAN Fingerprints
Ning Yu, Larry S. Davis, Mario Fritz; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 7556-7566
http://openaccess.thecvf.com/content_ICCV_2019/html/Yu_Attributing_Fake_Images_to_GANs_Learning_and_Analyzing_GAN_Fingerprints_ICCV_2019_paper.html

CIIDefence: Defeating Adversarial Attacks by Fusing Class-Specific Image Inpainting and Image Denoising
Puneet Gupta, Esa Rahtu; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 6708-6717
http://openaccess.thecvf.com/content_ICCV_2019/html/Gupta_CIIDefence_Defeating_Adversarial_Attacks_by_Fusing_Class-Specific_Image_Inpainting_and_ICCV_2019_paper.html

Multi-Adversarial Faster-RCNN for Unrestricted Object Detection
Zhenwei He, Lei Zhang; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 6668-6677
http://openaccess.thecvf.com/content_ICCV_2019/html/He_Multi-Adversarial_Faster-RCNN_for_Unrestricted_Object_Detection_ICCV_2019_paper.html

Bilateral Adversarial Training: Towards Fast Training of More Robust Models Against Adversarial Attacks
Jianyu Wang, Haichao Zhang; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 6629-6638
http://openaccess.thecvf.com/content_ICCV_2019/html/Wang_Bilateral_Adversarial_Training_Towards_Fast_Training_of_More_Robust_Models_ICCV_2019_paper.html

Self-Training and Adversarial Background Regularization for Unsupervised Domain Adaptive One-Stage Object Detection
Seunghyeon Kim, Jaehoon Choi, Taekyung Kim, Changick Kim; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 6092-6101
http://openaccess.thecvf.com/content_ICCV_2019/html/Kim_Self-Training_and_Adversarial_Background_Regularization_for_Unsupervised_Domain_Adaptive_One-Stage_ICCV_2019_paper.html

Adversarial Representation Learning for Text-to-Image Matching
Nikolaos Sarafianos, Xiang Xu, Ioannis A. Kakadiaris; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 5814-5824
http://openaccess.thecvf.com/content_ICCV_2019/html/Sarafianos_Adversarial_Representation_Learning_for_Text-to-Image_Matching_ICCV_2019_paper.html

Once a MAN: Towards Multi-Target Attack via Learning Multi-Target Adversarial Network Once
Jiangfan Han, Xiaoyi Dong, Ruimao Zhang, Dongdong Chen, Weiming Zhang, Nenghai Yu, Ping Luo, Xiaogang Wang; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 5158-5167
http://openaccess.thecvf.com/content_ICCV_2019/html/Han_Once_a_MAN_Towards_Multi-Target_Attack_via_Learning_Multi-Target_Adversarial_ICCV_2019_paper.html

Targeted Mismatch Adversarial Attack: Query With a Flower to Retrieve the Tower
Giorgos Tolias, Filip Radenovic, Ondrej Chum; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 5037-5046
http://openaccess.thecvf.com/content_ICCV_2019/html/Tolias_Targeted_Mismatch_Adversarial_Attack_Query_With_a_Flower_to_Retrieve_ICCV_2019_paper.html

Guessing Smart: Biased Sampling for Efficient Black-Box Adversarial Attacks
Thomas Brunner, Frederik Diehl, Michael Truong Le, Alois Knoll; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 4958-4966
http://openaccess.thecvf.com/content_ICCV_2019/html/Brunner_Guessing_Smart_Biased_Sampling_for_Efficient_Black-Box_Adversarial_Attacks_ICCV_2019_paper.html

Defending Against Universal Perturbations With Shared Adversarial Training
Chaithanya Kumar Mummadi, Thomas Brox, Jan Hendrik Metzen; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 4928-4937
http://openaccess.thecvf.com/content_ICCV_2019/html/Mummadi_Defending_Against_Universal_Perturbations_With_Shared_Adversarial_Training_ICCV_2019_paper.html

Universal Perturbation Attack Against Image Retrieval
Jie Li, Rongrong Ji, Hong Liu, Xiaopeng Hong, Yue Gao, Qi Tian; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 4899-4908
http://openaccess.thecvf.com/content_ICCV_2019/html/Li_Universal_Perturbation_Attack_Against_Image_Retrieval_ICCV_2019_paper.html

A Geometry-Inspired Decision-Based Attack
Yujia Liu, Seyed-Mohsen Moosavi-Dezfooli, Pascal Frossard; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 4890-4898
http://openaccess.thecvf.com/content_ICCV_2019/html/Liu_A_Geometry-Inspired_Decision-Based_Attack_ICCV_2019_paper.html

Improving Adversarial Robustness via Guided Complement Entropy
Hao-Yun Chen, Jhao-Hong Liang, Shih-Chieh Chang, Jia-Yu Pan, Yu-Ting Chen, Wei Wei, Da-Cheng Juan; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 4881-4889
http://openaccess.thecvf.com/content_ICCV_2019/html/Chen_Improving_Adversarial_Robustness_via_Guided_Complement_Entropy_ICCV_2019_paper.html

The LogBarrier Adversarial Attack: Making Effective Use of Decision Boundary Information
Chris Finlay, Aram-Alexandre Pooladian, Adam Oberman; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 4862-4870
http://openaccess.thecvf.com/content_ICCV_2019/html/Finlay_The_LogBarrier_Adversarial_Attack_Making_Effective_Use_of_Decision_Boundary_ICCV_2019_paper.html

Scalable Verified Training for Provably Robust Image Classification
Sven Gowal, Krishnamurthy (Dj) Dvijotham, Robert Stanforth, Rudy Bunel, Chongli Qin, Jonathan Uesato, Relja Arandjelovic, Timothy Mann, Pushmeet Kohli; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 4842-4851
http://openaccess.thecvf.com/content_ICCV_2019/html/Gowal_Scalable_Verified_Training_for_Provably_Robust_Image_Classification_ICCV_2019_paper.html

Physical Adversarial Textures That Fool Visual Object Tracking
Rey Reza Wiyatno, Anqi Xu; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 4822-4831
http://openaccess.thecvf.com/content_ICCV_2019/html/Wiyatno_Physical_Adversarial_Textures_That_Fool_Visual_Object_Tracking_ICCV_2019_paper.html

Hilbert-Based Generative Defense for Adversarial Examples
Yang Bai, Yan Feng, Yisen Wang, Tao Dai, Shu-Tao Xia, Yong Jiang; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 4784-4793
http://openaccess.thecvf.com/content_ICCV_2019/html/Bai_Hilbert-Based_Generative_Defense_for_Adversarial_Examples_ICCV_2019_paper.html

Semantic Adversarial Attacks: Parametric Transformations That Fool Deep Classifiers
Ameya Joshi, Amitangshu Mukherjee, Soumik Sarkar, Chinmay Hegde; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 4773-4783
http://openaccess.thecvf.com/content_ICCV_2019/html/Joshi_Semantic_Adversarial_Attacks_Parametric_Transformations_That_Fool_Deep_Classifiers_ICCV_2019_paper.html

Enhancing Adversarial Example Transferability With an Intermediate Level Attack
Qian Huang, Isay Katsman, Horace He, Zeqi Gu, Serge Belongie, Ser-Nam Lim; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 4733-4742
http://openaccess.thecvf.com/content_ICCV_2019/html/Huang_Enhancing_Adversarial_Example_Transferability_With_an_Intermediate_Level_Attack_ICCV_2019_paper.html

Sparse and Imperceivable Adversarial Attacks
Francesco Croce, Matthias Hein; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 4724-4732
http://openaccess.thecvf.com/content_ICCV_2019/html/Croce_Sparse_and_Imperceivable_Adversarial_Attacks_ICCV_2019_paper.html

Be Your Own Teacher: Improve the Performance of Convolutional Neural Networks via Self Distillation
Linfeng Zhang, Jiebo Song, Anni Gao, Jingwei Chen, Chenglong Bao, Kaisheng Ma; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 3713-3722
http://openaccess.thecvf.com/content_ICCV_2019/html/Zhang_Be_Your_Own_Teacher_Improve_the_Performance_of_Convolutional_Neural_ICCV_2019_paper.html

Adversarial Defense by Restricting the Hidden Space of Deep Neural Networks
Aamir Mustafa, Salman Khan, Munawar Hayat, Roland Goecke, Jianbing Shen, Ling Shao; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 3385-3394
http://openaccess.thecvf.com/content_ICCV_2019/html/Mustafa_Adversarial_Defense_by_Restricting_the_Hidden_Space_of_Deep_Neural_ICCV_2019_paper.html

Adversarial Feedback Loop
Firas Shama, Roey Mechrez, Alon Shoshan, Lihi Zelnik-Manor; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 3205-3214
http://openaccess.thecvf.com/content_ICCV_2019/html/Shama_Adversarial_Feedback_Loop_ICCV_2019_paper.html

Siamese Networks: The Tale of Two Manifolds
Soumava Kumar Roy, Mehrtash Harandi, Richard Nock, Richard Hartley; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 3046-3055
http://openaccess.thecvf.com/content_ICCV_2019/html/Roy_Siamese_Networks_The_Tale_of_Two_Manifolds_ICCV_2019_paper.html

Universal Adversarial Perturbation via Prior Driven Uncertainty Approximation
Hong Liu, Rongrong Ji, Jie Li, Baochang Zhang, Yue Gao, Yongjian Wu, Feiyue Huang; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 2941-2949
http://openaccess.thecvf.com/content_ICCV_2019/html/Liu_Universal_Adversarial_Perturbation_via_Prior_Driven_Uncertainty_Approximation_ICCV_2019_paper.html

Adversarial Defense via Learning to Generate Diverse Attacks
Yunseok Jang, Tianchen Zhao, Seunghoon Hong, Honglak Lee; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 2740-2749
http://openaccess.thecvf.com/content_ICCV_2019/html/Jang_Adversarial_Defense_via_Learning_to_Generate_Diverse_Attacks_ICCV_2019_paper.html

Memorizing Normality to Detect Anomaly: Memory-Augmented Deep Autoencoder for Unsupervised Anomaly Detection
Dong Gong, Lingqiao Liu, Vuong Le, Budhaditya Saha, Moussa Reda Mansour, Svetha Venkatesh, Anton van den Hengel; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 1705-1714
http://openaccess.thecvf.com/content_ICCV_2019/html/Gong_Memorizing_Normality_to_Detect_Anomaly_Memory-Augmented_Deep_Autoencoder_for_Unsupervised_ICCV_2019_paper.html

Anomaly Detection in Video Sequence With Appearance-Motion Correspondence
Trong-Nguyen Nguyen, Jean Meunier; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 1273-1283
http://openaccess.thecvf.com/content_ICCV_2019/html/Nguyen_Anomaly_Detection_in_Video_Sequence_With_Appearance-Motion_Correspondence_ICCV_2019_paper.html

Bit-Flip Attack: Crushing Neural Network With Progressive Bit Search
Adnan Siraj Rakin, Zhezhi He, Deliang Fan; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 1211-1220
http://openaccess.thecvf.com/content_ICCV_2019/html/Rakin_Bit-Flip_Attack_Crushing_Neural_Network_With_Progressive_Bit_Search_ICCV_2019_paper.html

Hiding Video in Audio via Reversible Generative Models
Hyukryul Yang, Hao Ouyang, Vladlen Koltun, Qifeng Chen; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 1100-1109
http://openaccess.thecvf.com/content_ICCV_2019/html/Yang_Hiding_Video_in_Audio_via_Reversible_Generative_Models_ICCV_2019_paper.html

Towards Adversarially Robust Object Detection
Haichao Zhang, Jianyu Wang; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 421-430
http://openaccess.thecvf.com/content_ICCV_2019/html/Zhang_Towards_Adversarially_Robust_Object_Detection_ICCV_2019_paper.html

Evaluating Robustness of Deep Image Super-Resolution Against Adversarial Attacks
Jun-Ho Choi, Huan Zhang, Jun-Hyuk Kim, Cho-Jui Hsieh, Jong-Seok Lee; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 303-311
http://openaccess.thecvf.com/content_ICCV_2019/html/Choi_Evaluating_Robustness_of_Deep_Image_Super-Resolution_Against_Adversarial_Attacks_ICCV_2019_paper.html

On the Design of Black-Box Adversarial Examples by Leveraging Gradient-Free Optimization and Operator Splitting Method
Pu Zhao, Sijia Liu, Pin-Yu Chen, Nghia Hoang, Kaidi Xu, Bhavya Kailkhura, Xue Lin; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 121-130
http://openaccess.thecvf.com/content_ICCV_2019/html/Zhao_On_the_Design_of_Black-Box_Adversarial_Examples_by_Leveraging_Gradient-Free_ICCV_2019_paper.html

==> large_key_encryption.tex <==
% !TEX root =  main.tex 

\section{Big-Key Encryption}


\nico{Make a reference and some discussion about cryptographic sensing and cryptographic phenomena in the natural world}

\nico{We make a connection between robust unlearnability and cryptography in the bounded retrieval model. Learning algorithm corresponds to bounded retrieval adversary}

\nico{Big-Key Encryption of Knowledge: Extractor which allows us to extract key from distinguisher, composes easier than IND-BRM}

In this Section, we provide definitions and constructions for a primitive we call \emph{big-Key Encryption}. Roughly speaking, space encryption schemes are encryption schemes where anyone in possession of a long random string $\witness$ will be able to decrypt ciphertexts $\ciph$ that were encrypted with respect to $\witness$ or a short commitment of it. The important aspect about this primitive is that even \emph{forgetting} a small fraction of $\witness$ will make it impossible to decrypt such a $\ciph$. In terms of compactness, we will require that the size of ciphertexts is independent of the size of the string $\witness$.

\nico{Being able to decrypt is a 'proof of storage' (somewhat different from proof of space)}

\begin{definition}
A big-key encryption scheme consists of 3 algorithms $(\Setup,\Enc,\Dec)$ with the following syntax.
\begin{itemize}
    \item $\Setup(1^\secp,\ell)$: Takes as input a security parameter $1^\secp$ and a size-parameter $\ell$ and outputs a public key $\pk$ and a secret key $\sk$.
    \item $\Enc(\pk,\mes)$: Takes as input a public key $\pk$ and a message $\mes$ and outputs a ciphertext $\ciph$
    \item $\Dec(\sk,\ciph)$: Takes as input a secret key $\sk$ and a ciphertext $\ciph$ and outputs a message $\mes'$.
\end{itemize}
Assume for simplicity that the message space is $\bin$. We require the following properties.
\begin{itemize}
    \item \textbf{Correctness}: It holds for every message $\mes$ that $\Dec(\sk,\Enc(\pk,\mes)) = \mes$, where $(\pk,\sk) \gets \Setup(1^\secp,\ell)$.
    \item \textbf{Compactness}: Secret keys $\sk$ are of size at most $\ell \cdot \secp$. Public keys $\pk$ and ciphertexts $\ciph$ are of size $\poly$ and in particular independent of $\ell$. Furthermore, we require that the runtime of $\Enc$ is also $\poly$ independent of $\ell$.
    \item \textbf{Incompressability Security}: In terms of security, we require that following. Let $\ell = \ell(\secp) = \poly$ and $\epsilon = \epsilon(\secp) \in (0,1]$. Let $\A = (\A_1,\A_2)$ be a PPT adversary consisting of two stages $\A_1$ and $\A_2$ such that $\A_1$ outputs a string $\tau$ of length at most $(1-\epsilon) \ell \cdot \secp$ and two messages $\mes_0$ and $\mes_1$. Consider the following experiment.
    \begin{description}
    \item[$\Exp_\A(\ell,\epsilon)$]:
    \begin{itemize}
        \item $(\pk,\sk) \gets \Setup(1^\secp,\ell)$
        \item Compute $(\tau,\mes_0,\mes_1) \gets \A_1(\pk,\sk)$
        \item Choose a bit $b \pick \bin$
        \item $\ciph^\ast \gets \Enc(\pk,\mes_b)$
        \item Compute $b' \gets \A_2(\pk,\tau,\ciph^\ast)$
        \item If $b' = b$ output 1, otherwise 0
    \end{itemize}
    \end{description}
    We say that a big-key encryption scheme $(\Setup,\Enc,\Dec)$ is indistinguishability-secure, if it holds for every PPT adversary $\A$ satifying the above constraints that
    \[
    \Pr[\Exp_\A(\ell,\epsilon) = 1] \leq \frac{1}{2} + \negl.
    \]
\end{itemize}
\end{definition}

\nico{Define private key analogues, construction idea: sender selects subset of a long list of keys, what is the sample entropy of a subset of keys given an arbitrary leak}

\subsection{A Construction in the Random Oracle Model}

\nico{We need a malleable construction}


We first provide a construction of a big-key encryption scheme in the random oracle model.

%The basic idea is simple. 

Let $\Hash: \bin^\secp \times \bin^\ell \to \bin^\secp$ be a hash function modelled as a random oracle. Let $(\Enc,\Dec)$ be a private key encryption scheme for which keys are uniformly random strings from $\bin^\secp$. Our scheme $\Pi' = (\Setup',\Enc',\Dec')$ is given as follows.

\begin{itemize}
    \item $\Setup'(1^\secp, \ell):$ Choose a uniformly random string $\key \pick \bin^\ell$.
    \item $\Enc'(\key,\mes)$: Choose a uniformly random $\seed \pick \bin^\secp$. Compute $\ciph \gets \Enc(\Hash(\seed,\key),\mes)$ and output $\ciph' \gets (\seed,\ciph)$.
    \item $\Dec'(\key,\ciph')$: Parse $\ciph' = (\seed,\ciph)$. Compute $\mes' \gets \Dec(\Hash(\seed,\key),\ciph)$ and output $\mes'$.
\end{itemize}

Correctness of $\Pi'$ follows immediately from the correctness of $(\Enc,\Dec)$ and the fact that $\Hash$ is deterministic. Moreover, it follows immediately that the ciphertext size is $\poly$, independent of $\ell$.

We now show that the scheme satisfies incompressability security.

\begin{theorem}
Assume that $(\Enc,\Dec)$ is a one-time secure private key encryption scheme and that $\Hash$ is a random oracle. Then the scheme $\Pi'$ satisfies incompressability security.
\end{theorem}


\begin{proof}
Fix a PPT adversary $\A$ and let $q = \poly$ be an upper bound on the sum of the number of queries $\A$ makes to the random oracle $\Hash$ and the number of queries $\A$ makes to the encryption oracle $\Enc'(\key,\cdot)$ in the second stage.

Consider the following hybrids.

\begin{itemize}
    \item Hybrid $\Hyb_0$: This is the real experiment.
    
    \item Hybrid $\Hyb_1$: This is identical to $\Hyb_0$, except that the experiment aborts if $\A$ queries $\Hash$ with seed $\seed^\ast$ in the first stage or if an encryption query in the second stage uses the seed $\seed^\ast$. 
    
    \item Hybrid $\Hyb_2$: Identical to $\Hyb_1$, except that the experiment aborts if $\A$ queries $\Hash$ on $\key$ in the second stage.
    
    \item Hybrid $\Hyb_3$: Identical to $\Hyb_2$, except that we compute the challenge ciphertext $\ciph^\ast$ by $\ciph^\ast \gets \Enc'(\key,0^\ast)$.
    
\end{itemize}

In $\Hyb_3$ the view of the adversary $\A$ is independent of the challenge bit $b$, consequently the advantage of $\A$ is 0 in $\Hyb_3$. We will now show indistinguishability of the hybrids.


\paragraph{$\Hyb_0 \to \Hyb_1$:}
We will now show that $\Hyb_0$ and $\Hyb_1$ are statistically close. Conditioned that $\A$ does not query $\Hash$ on $\seed^\ast$ in stage 1 the two experiments are identically distributed. As $\seed^\ast$ is only chosen in stage 2 and $\seed^\ast$ is distributed uniformly random on $\bin^\secp$, every single (adversarially chosen) seed $\seed'$ used in the first stage has a probability of colliding with $\seed^\ast$ of $2^{-\secp}$. Likewise, since the seeds $\seed''$ used by the encryption oracle in the second stage are chosen uniformly at random from $\bin^\secp$, every $\seed''$ has a probability of colliding with $\seed^\ast$ of $2^{-\secp}$. Consequently, it follows by a union-bound that the probability that and abort happens is at most $q \cdot 2^{-\secp}$, which is negligible. Consequently, the statistical distance between $\Hyb_0$ and $\Hyb_1$ is $q \cdot 2^{-\secp}$.

\paragraph{$\Hyb_1 \to \Hyb_2$:}
We will now show that $\Hyb_1$ and $\Hyb_2$ are statistically close. Note first that conditioned that $\A$ does not query its oracle $\Hash$ with $\key$ in stage 2, the two experiments are identically distributed. We will therefore bound the probability that $\A$ queries $\Hash$ with key in stage 2.

We will do this by showing that such an $\A$ would lead to a compression and decompression algorithm for the uniformly random string $\key$, which is information-theoretically impossible by Lemma \ref{}.  

\paragraph{$\Hyb_2 \to \Hyb_3$:}
We will now show that $\Hyb_2$ and $\Hyb_3$ are (computationally) indistinguishable given that the encryption scheme $(\Enc,\Dec)$ is one-time secure. First note that we have ensured that in $\Hyb_2$ the derived key $\Hash(\seed^\ast,\key)$ is only used to encrypt the challenge message. Secondly, in this experiment $\A$ cannot obtain $\Hash(\seed^\ast,\key)$ via a call to the random oracle $\Hash$. Thus, $\Hash(\seed^\ast,\key)$ is only used by $\Enc$, which allows us to mount a reduction to the one-time security of $(\Enc,\Dec)$ as follows.

The reduction $\mathcal{R}$...

\nico{Todo}

\end{proof}








% In this Section we will construct a private key encryption scheme with large and incompressible secret keys. In the next Section, we will use such a scheme construct a learning task which is robustly learnable for any fixed metric, but provably not robustly learnable in several metrics simultaneously.


% \nico{Construction is identical to that of private key encryption with resilience against key leakage. }


% Let $\Pi' = (\Enc',\Dec')$ be a private key encryption scheme with uniformly random keys in $\bin^\secp$ and $\Ext: \bin^\secp \times \bin^\ell \to \bin^\secp$ be a (seeded) randomness extractor. We will construct a private key encryption scheme $\Pi = (\KeyGen,\Enc,\Dec)$ which has large and incompressible secret keys. We will make the keysize $\ell$ an explicit input to the key generation algorithm. The scheme $\Pi = (\KeyGen,\Enc,\Dec)$ is given as follows.

% \begin{description}
% \item[$\KeyGen(1^\secp,\ell)$]: Choose a uniformly random $\key \pick \bin^\ell$ and output $\key$.

% \item[$\Enc(\key,\mes)$]: Choose a uniformly random seed $\seed \pick \bin^\secp$ and compute $\key' \gets \Ext(\seed,\key)$. Output $\ciph \gets (\seed,\Enc'(\key',\mes))$.

% \item[$\Dec(\key,\ciph)$]: Parse $\ciph$ as $\ciph = (\seed,\ciph')$. Compute $\key' \gets \Ext(\seed,\key)$ and compute $\mes \gets \Dec'(\key',\ciph')$.
% \end{description}

% Correctness of this scheme follows immediately from the correctness of $\Pi$. We will now show that this scheme is secure even under partial key leakage.

% \nico{$\Pi'$ can be a bit encryption scheme and we can reuse the seed $\seed$ across many ciphertexts}

% \begin{theorem}
% Assume that $\Pi' = (\Enc',\Dec')$ is a CPA secure encryption scheme and that $\Ext$ is a $(k,\eps)$ average-case extractor. Then $\Pi$ is CPA secure under $n - k$ bits of leakage.
% \end{theorem}

% \begin{proof}
% Fix a PPT adversary $\A$ and let $q$ be a polynomial upper bound on the number of encryption queries that $\A$ makes. 
% Let $\ciph^\ast \gets \Enc(\key,\mes_b)$ be the challenge ciphertext in the lCPA experiment and assume that Consider the following hybrids.

% \begin{itemize}
%     \item Hybrid $\Hyb_0$: This is the real experiment.
%     \item Hybrid $\Hyb_i$ for $i = 1,\dots,q$: This is identical to the previous hybrid, except that in encryption query $i$ we replace $\key'_i \gets \Ext(\seed_i,\key)$ by a uniformly random $\key''_i \pick \bin^\secp$.
    
% \end{itemize}


% \end{proof}


==> t-gnuplot-lua-tikz.tex <==
%%
%%  ConTeXt wrapper for gnuplot-tikz style file
%%
\usemodule[tikz]

\usetikzlibrary[arrows,patterns,plotmarks,backgrounds]

\edef\tikzatcode{\the\catcode`\@}
\edef\tikzbarcode{\the\catcode`\|}
\edef\tikzexclaimcode{\the\catcode`\!}
\catcode`\@=11
\catcode`\|=12
\catcode`\!=12

\input gnuplot-lua-tikz-common.tex

\catcode`\@=\tikzatcode
\catcode`\|=\tikzbarcode
\catcode`\!=\tikzexclaimcode

\endinput

